Dynamic Cheatsheet: Test-Time Learning with Adaptive Memory

Despite their impressive performance on complex tasks, current language models (LMs) typically operate in a vacuum: Each input query is processed separately, without retaining insights from previous attempts. Here, we present Dynamic Cheatsheet (DC), a lightweight framework that endows a black-box LM with a persistent, evolving memory. Rather than repeatedly re-discovering or re-committing the same solutions and mistakes, DC enables models to store and reuse accumulated strategies, code snippets, and general problem-solving insights at inference time. This test-time learning enhances performance substantially across a range of tasks without needing explicit ground-truth labels or human feedback. Leveraging DC, Claude 3.5 Sonnet's accuracy more than doubled on AIME math exams once it began retaining algebraic insights across questions. Similarly, GPT-4o's success rate on Game of 24 increased from 10% to 99% after the model discovered and reused a Python-based solution. In tasks prone to arithmetic mistakes, such as balancing equations, DC enabled GPT-4o and Claude to reach near-perfect accuracy by recalling previously validated code, whereas their baselines stagnated around 50%. Beyond arithmetic challenges, DC yields notable accuracy gains on knowledge-demanding tasks. Claude achieved a 9% improvement in GPQA-Diamond and an 8% boost on MMLU-Pro problems. Crucially, DC's memory is self-curated, focusing on concise, transferable snippets rather than entire transcript. Unlike finetuning or static retrieval methods, DC adapts LMs' problem-solving skills on the fly, without modifying their underlying parameters. Overall, our findings present DC as a promising approach for augmenting LMs with persistent memory, bridging the divide between isolated inference events and the cumulative, experience-driven learning characteristic of human cognition.

==> macros_legacy.tex <==
\definecolor{battleshipgrey}{rgb}{0.3, 0.3, 0.3}
\definecolor{brilliantrose}{rgb}{1.0, 0.33, 0.64}
\definecolor{americanrose}{rgb}{1.0, 0.01, 0.24}
\definecolor{jweigreen}{rgb}{0,0.45,0.24}
\definecolor{bluegray}{rgb}{0.1, 0.1, 0.4}
\definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
\definecolor{blanchedalmond}{rgb}{1.0, 0.92, 0.8}
\definecolor{atomictangerine}{rgb}{1.0, 0.6, 0.4}
\definecolor{chocolate(web)}{rgb}{0.82, 0.41, 0.12}
\definecolor{bananayellow}{rgb}{1.0, 0.88, 0.21}
\definecolor{goldenbrown}{rgb}{0.6, 0.4, 0.08}
\definecolor{aliceblue}{rgb}{0.94, 0.97, 1.0}
\definecolor{beige}{rgb}{0.96, 0.96, 0.86}
\definecolor{babyblue}{rgb}{0.54, 0.81, 0.94}
\definecolor{camel}{rgb}{0.76, 0.6, 0.42}
\definecolor{cinnamon}{rgb}{0.82, 0.41, 0.12}
\definecolor{deepskyblue}{rgb}{0.0, 0.75, 1.0}
\definecolor{frenchblue}{rgb}{0.0, 0.45, 0.73}
\definecolor{classicrose}{rgb}{0.98, 0.8, 0.91}
\definecolor{frenchrose}{rgb}{0.96, 0.29, 0.54}
\definecolor{frenchlilac}{rgb}{0.53, 0.38, 0.56}
\definecolor{frenchbeige}{rgb}{0.65, 0.48, 0.36}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}
\definecolor{dartmouthgreen}{rgb}{0.05, 0.5, 0.06}
\definecolor{turquoisegreen}{rgb}{0.63, 0.84, 0.71}
\definecolor{darkseagreen}{rgb}{0.56, 0.74, 0.56}
\definecolor{columbiablue}{rgb}{0.61, 0.87, 1.0}
\definecolor{rufous}{rgb}{0.66, 0.11, 0.03}
\definecolor{cyan(process)}{rgb}{0.0, 0.72, 0.92}
\definecolor{crimsonglory}{rgb}{0.75, 0.0, 0.2}
\definecolor{yaleblue}{rgb}{0.06, 0.3, 0.57}

\newcommand{\applegreen}[1]{{\color{applegreen}{#1}}}
\newcommand{\battleshipgrey}[1]{{\color{battleshipgrey}{#1}}}
\newcommand{\americanrose}[1]{{\color{americanrose}{#1}}}
\newcommand{\jweigreen}[1]{{\color{jweigreen}{#1}}}
\newcommand{\darkgreen}[1]{{\color{ao(english)}{#1}}}
\newcommand{\aliceblue}[1]{{\color{aliceblue}{#1}}}
\newcommand{\beige}[1]{{\color{beige}{#1}}}
\newcommand{\babyblue}[1]{{\color{babyblue}{#1}}}
\newcommand{\camel}[1]{{\color{camel}{#1}}}
\newcommand{\cinnamon}[1]{{\color{cinnamon}{#1}}}
\newcommand{\crimsonglory}[1]{{\color{crimsonglory}{#1}}}
\newcommand{\cyan}[1]{{\color{cyan}{#1}}}
\newcommand{\deepskyblue}[1]{{\color{deepskyblue}{#1}}}
\newcommand{\frenchblue}[1]{{\color{frenchblue}{#1}}}
\newcommand{\classicrose}[1]{{\color{classicrose}{#1}}}
\newcommand{\frenchrose}[1]{{\color{frenchrose}{#1}}}
\newcommand{\frenchlilac}[1]{{\color{frenchlilac}{#1}}}
\newcommand{\frenchbeige}[1]{{\color{frenchbeige}{#1}}}
\newcommand{\dartmouthgreen}[1]{{\color{dartmouthgreen}{#1}}}
\newcommand{\turquoisegreen}[1]{{\color{turquoisegreen}{#1}}}
\newcommand{\darkseagreen}[1]{{\color{darkseagreen}{#1}}}
\newcommand{\rufous}[1]{{\color{rufous}{#1}}}
\newcommand{\yaleblue}[1]{{\color{yaleblue}{#1}}}

\newcommand{\sg}[1]{\draftcomment{\textcolor{orange}{\small [#1]$_{\textrm{sg}}$}}}

\newcommand{\atk}[1]{{\textcolor{blue}{\small [#1]$_{\textrm{atk}}$}}}

\usepackage{tcolorbox}

\newcommand{\Commenttt}[1]{\Comment{\textcolor{gray}{\footnotesize\textit{#1}}}}


